Measuring the Effect of Transcription Noise on Downstream Language Understanding Tasks

With the increasing prevalence of recorded human speech, spoken language understanding (SLU) is essential for its efficient processing. In order to process the speech, it is commonly transcribed using automatic speech recognition technology. This speech-to-text transition introduces errors into the transcripts, which subsequently propagate to downstream NLP tasks, such as dialogue summarization. While it is known that transcript noise affects downstream tasks, a systematic approach to analyzing its effects across different noise severities and types has not been addressed. We propose a configurable framework for assessing task models in diverse noisy settings, and for examining the impact of transcript-cleaning techniques. The framework facilitates the investigation of task model behavior, which can in turn support the development of effective SLU solutions. We exemplify the utility of our framework on three SLU tasks and four task models, offering insights regarding the effect of transcript noise on tasks in general and models in particular. For instance, we find that task models can tolerate a certain level of noise, and are affected differently by the types of errors in the transcript.

==> figures/framework_full.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth, trim=102 225 118 101, clip]{figures/framework_full_img.pdf}
    \caption{The framework for assessing \ENDow{}, where each component in the pipeline is given in the input configuration. As a result of the pipeline, we can analyze the behavior of the task model at $k+2$ different levels of noise, as represented by line $l_0$. Additionally, the corresponding line $l_j$ of cleaning technique $j$ can be compared against $l_0$ to produce a final cleaning effectiveness score, comparable to other cleaning techniques.}
    \label{fig_framework}
\end{figure*}

==> tables/scores_noclean.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|cc|cc|cc|cc}
    \toprule
 & \multicolumn{2}{c|}{Mistral} & \multicolumn{2}{c|}{Llama3} & \multicolumn{2}{c|}{Llama3.1} & \multicolumn{2}{c|}{GPT4oMini} \\
    Task | Metric & AUC & NTP & AUC & NTP & AUC & NTP & AUC & NTP \\
    \midrule
    QMSum | PW-Rank &     \textbf{5.817} \small{± 0.321} & 0.195 &     5.811 \small{± 0.331} & 0.070 &     5.746 \small{± 0.312} & 0.249 &     5.627 \small{± 0.280} & 0.297 \\
    \midrule
    QAConv | Fuzzy &     39.080 \small{± 1.241} & 0.341 &     37.331 \small{± 1.217} & 0.302 &     49.466 \small{± 1.288} & 0.051 &     \textbf{49.992} \small{± 1.286} & 0.214 \\
    \midrule
    MRDA | Mac-$F_1$ &     0.110 \small{± 0.019} & 0.560 &     0.149 \small{± 0.028} & 0.615 &     0.140 \small{± 0.028} & 0.709 &     \textbf{0.193} \small{± 0.032} & 0.439 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{The area-under-the-curve (AUC; with margin of error at 95\% confidence level) and the noise-tolerance point (NTP) of the experimented task models on the three tasks (summarization, question-answering and dialog-act classification). The highest AUC in each row is in bold. The scores correspond to the graphs in \autoref{fig_noclean_graphs}, where a more in-depth examination can be conducted. The full table (for all metrics) is in the Appendix, \autoref{tab_scores_noclean_all}.}
    \label{tab_scores_noclean}
\end{table*}
